Latent Fact-Checking: Detecting Misinformation through Activation Engineering

The proliferation of misinformation online has driven demand for scalable detection systems. While most existing approaches rely on surface-level linguistic features or external knowledge retrieval, we examine truthfulness as a geometric property of a language model's representation space. We introduce a misinformation detection framework grounded in activation engineering, which leverages the latent geometry of transformer models. Our approach elicits a misinformation direction in the residual stream by contrasting activations from paired truthful and false statements, following the difference-in-means principle of Contrastive Activation Addition (CAA). At inference time, the last-token activation of an unseen claim is projected onto this direction, and the projected representation is fed to an Multilayer Perceptron (MLP) for classification. The procedure requires no fine-tuning of the backbone model, no external evidence retrieval, and no task-specific supervision beyond the contrastive pairs used to estimate the direction. We evaluate the method across 11 models from the Gemma, Llama, and Qwen families, ranging from 270M to 12B parameters, on three fact-checking benchmarks: AVeriTeC, LIAR, and FACTors. The falsehood direction is recoverable across model scales and architectural families, and last-token projection matches or surpasses zero-shot and few-shot prompting baselines on LIAR and FACTors, with the largest gains observed for smaller models. Performance on AVeriTeC is more limited, which we attribute to its evidence-grounded labeling scheme. These findings provide evidence that truthfulness is a structured, linearly separable concept in the latent space of pretrained language models, and point toward interpretability-driven misinformation detection as a practical complement to retrieval-based pipelines. The code is available on https://github.com/Malta-Lab/LaFaCt.

==> figures/lafact_pipeline.tex <==

% ── Colour palette ──────────────────────────────────────────────────────────
\definecolor{clrDataset}  {RGB}{236,231,248}   % soft purple  – data / input
\definecolor{clrDatasetB} {RGB}{108, 86,163}
\definecolor{clrPrompt}   {RGB}{225,243,252}   % soft blue    – prompt construction
\definecolor{clrPromptB}  {RGB}{ 52,144,196}
\definecolor{clrLLM}      {RGB}{220,240,230}   % soft teal    – frozen LLM
\definecolor{clrLLMB}     {RGB}{ 38,139, 90}
\definecolor{clrVector}   {RGB}{255,237,213}   % soft amber   – vector ops
\definecolor{clrVectorB}  {RGB}{200,120,  0}
\definecolor{clrLayer}    {RGB}{255,228,225}   % soft coral   – layer selection
\definecolor{clrLayerB}   {RGB}{196, 72, 54}
\definecolor{clrMLP}      {RGB}{228,245,220}   % soft green   – classifier
\definecolor{clrMLPB}     {RGB}{ 74,150, 46}
\definecolor{clrPhase}    {RGB}{245,245,245}   % phase bg
\definecolor{clrDiv}      {RGB}{170,170,170}

% ── Node styles ─────────────────────────────────────────────────────────────
\tikzset{
  base/.style={
    rectangle, rounded corners=4pt,
    minimum width=2.8cm, minimum height=0.95cm,
    align=center, font=\small,
    inner sep=5pt, text width=2.6cm,
    line width=0.5pt
  },
  dataset/.style ={base, fill=clrDataset,  draw=clrDatasetB},
  prompt/.style  ={base, fill=clrPrompt,   draw=clrPromptB },
  llm/.style     ={base, fill=clrLLM,      draw=clrLLMB    },
  vector/.style  ={base, fill=clrVector,   draw=clrVectorB },
  layersel/.style={base, fill=clrLayer,    draw=clrLayerB  },
  mlp/.style     ={base, fill=clrMLP,      draw=clrMLPB    },
  arrow/.style   ={-{Stealth[length=5pt,width=4pt]}, line width=0.7pt, color=clrDiv},
  darrow/.style  ={arrow, dashed},
  label/.style   ={font=\scriptsize\itshape, text=gray},
  phase/.style   ={rectangle, rounded corners=6pt,
                   fill=clrPhase, draw=clrDiv,
                   line width=0.4pt, dashed, inner sep=12pt},
  phaselabel/.style={font=\footnotesize\bfseries, text=clrDiv,
                     rotate=90, anchor=south}
}

% ════════════════════════════════════════════════════════════════════════════
%
%  LaFaCt pipeline – two-row layout
%
%  Row A (top):    Direction estimation sub-phase
%                  Dataset → A/B prompts → Frozen LLM (all ℓ) → Activations h±
%                  → Diff-of-means v^(ℓ) → Normalise v̂^(ℓ)
%
%  Row B (middle): Layer-selection sub-phase
%                  Dataset (plain) → Frozen LLM (all ℓ) → Activations h
%                  → Project onto v̂^(ℓ) [each ℓ] → MLP probe → Layer sel ℓ*
%                  → MLP retrain on D_tr∪D_val
%
%  Row C (bottom): Inference phase
%                  New claim → Frozen LLM (layer ℓ*) → Activation h^(ℓ*)
%                  → Project onto v̂^(ℓ*) → MLP → Prediction
%
% ════════════════════════════════════════════════════════════════════════════

\begin{tikzpicture}[node distance=0.7cm and 0.65cm]

% ────────────────────────────────────────────────────────────────────────────
%  ROW A – Direction estimation
% ────────────────────────────────────────────────────────────────────────────

\node[dataset] (dataset)
  {\textbf{Dataset}\\$\mathcal{D}{=}\{(s_i,y_i)\}$};

\node[prompt,  right=of dataset] (abprompt)
  {\textbf{A/B prompts}\\$p_i^{+},\,p_i^{-}$};

\node[llm,     right=of abprompt] (llmdir)
  {\textbf{Frozen LLM}\\all layers $\ell$};

\node[vector,  right=of llmdir] (actpm)
  {\textbf{Activations}\\$\mathbf{h}_i^{(\ell)+},\,\mathbf{h}_i^{(\ell)-}$};

\node[vector,  right=of actpm] (diffmeans)
  {\textbf{Diff.\ of means}\\
   $\mathbf{v}^{(\ell)}{=}\overline{\mathbf{h}^+}{-}\overline{\mathbf{h}^-}$};

\node[vector,  right=of diffmeans] (normvec)
  {\textbf{Norm.\ direction}\\
   $\hat{\mathbf{v}}^{(\ell)}{=}\dfrac{\mathbf{v}^{(\ell)}}{\|\mathbf{v}^{(\ell)}\|_2}$};

% Row A arrows
\draw[arrow] (dataset)   -- (abprompt)
  node[label, midway, above] {A/B template};
\draw[arrow] (abprompt)  -- (llmdir);
\draw[arrow] (llmdir)    -- (actpm)
  node[label, midway, above] {\texttt{LastTok}};
\draw[arrow] (actpm)     -- (diffmeans);
\draw[arrow] (diffmeans) -- (normvec);

% ────────────────────────────────────────────────────────────────────────────
%  ROW B – Layer selection + MLP retrain
% ────────────────────────────────────────────────────────────────────────────

\node[dataset,  below=2.2cm of dataset] (datasetB)
  {\textbf{Dataset}\\$\mathcal{D}{=}\{(s_i,y_i)\}$};

\node[llm,      right=of datasetB] (llmsel)
  {\textbf{Frozen LLM}\\all layers $\ell$};

\node[vector,   right=of llmsel] (actplain)
  {\textbf{Activations}\\$\mathbf{h}_i^{(\ell)}$ (plain)};

\node[vector,   right=of actplain] (projsel)
  {\textbf{Projection}\\
   $\mathbf{z}_i^{(\ell)}{=}(\mathbf{h}_i^{(\ell)}{\cdot}\hat{\mathbf{v}}^{(\ell)})\hat{\mathbf{v}}^{(\ell)}$};

\node[layersel, right=of projsel] (layersel)
  {\textbf{Layer selection}\\
   $\ell^*{=}\arg\max_\ell\,\mathrm{Acc}(\mathcal{D}_\mathrm{val})$};

\node[mlp,      right=of layersel] (mlptrain)
  {\textbf{MLP retrain}\\
   on $\mathcal{D}_\mathrm{tr}{\cup}\mathcal{D}_\mathrm{val}$\\
   at $\ell^*$};

% Row B arrows
\draw[arrow] (datasetB) -- (llmsel)
  node[label, midway, above] {no template};
\draw[arrow] (llmsel)   -- (actplain)
  node[label, midway, above] {\texttt{LastTok}};
\draw[arrow] (actplain) -- (projsel);
\draw[arrow] (projsel)  -- (layersel)
  node[label, midway, above] {MLP probe};
\draw[arrow] (layersel) -- (mlptrain)
  node[label, midway, above] {select $\ell^*$};

% v̂^(ℓ) flows from Row A into Row B projection
% Route: normvec.south → down between rows → left → projsel.north
\draw[darrow, clrVectorB]
  (normvec.south) -- ++(0,-0.8)
    -| (projsel.north)
  node[label, pos=0.6, below right=0pt and 2pt] {$\hat{\mathbf{v}}^{(\ell)}$};

% ────────────────────────────────────────────────────────────────────────────
%  ROW C – Inference
% ────────────────────────────────────────────────────────────────────────────

\node[dataset,  below=2.2cm of datasetB] (newclaim)
  {\textbf{New claim}\\$s$ (raw text)};

\node[llm,      right=of newclaim] (llminf)
  {\textbf{Frozen LLM}\\layer $\ell^*$};

\node[vector,   right=of llminf] (actinf)
  {\textbf{Activation}\\$\mathbf{h}^{(\ell^*)}$};

\node[vector,   right=of actinf] (projinf)
  {\textbf{Projection}\\
   $\mathbf{z}^{(\ell^*)}{=}(\mathbf{h}^{(\ell^*)}{\cdot}\hat{\mathbf{v}}^{(\ell^*)})\hat{\mathbf{v}}^{(\ell^*)}$};

\node[mlp,      right=of projinf] (mlpinf)
  {\textbf{MLP}\\$\hat{y}{=}\mathrm{MLP}(\mathbf{z}^{(\ell^*)})$};

\node[dataset,  right=of mlpinf] (pred)
  {\textbf{Prediction}\\$\hat{y}{\in}\{\textit{true},\textit{false}\}$};

% Row C arrows
\draw[arrow] (newclaim) -- (llminf)
  node[label, midway, above] {no template};
\draw[arrow] (llminf)   -- (actinf)
  node[label, midway, above] {\texttt{LastTok}};
\draw[arrow] (actinf)   -- (projinf);
\draw[arrow] (projinf)  -- (mlpinf);
\draw[arrow] (mlpinf)   -- (pred);

% ────────────────────────────────────────────────────────────────────────────
%  CROSS-PHASE DASHED TRANSFERS
% ────────────────────────────────────────────────────────────────────────────

% Normalised direction at ℓ* → inference projection
% Route: normvec.east → far right bus → down → projinf.east
\draw[darrow, clrVectorB]
  (normvec.east) -- ++(0.5,0)
    -- ++(0,-6.8)
    -| (projinf.east)
  node[label, pos=0.5, right=2pt] {$\hat{\mathbf{v}}^{(\ell^*)}$};

% MLP weights → inference MLP
\draw[darrow, clrMLPB]
  (mlptrain.south) -- ++(0,-0.4)
    -| (mlpinf.north)
  node[label, pos=0.3, right=2pt] {weights};

% ────────────────────────────────────────────────────────────────────────────
%  PHASE BACKGROUNDS
% ────────────────────────────────────────────────────────────────────────────
\begin{scope}[on background layer]
  \node[phase,
        fit=(dataset)(abprompt)(llmdir)(actpm)(diffmeans)(normvec)
            (datasetB)(llmsel)(actplain)(projsel)(layersel)(mlptrain),
        label={[phaselabel]left:\textsc{Training}}] (trainbox) {};

  \node[phase,
        fit=(newclaim)(llminf)(actinf)(projinf)(mlpinf)(pred),
        label={[phaselabel]left:\textsc{Inference}}] {};
\end{scope}

% ────────────────────────────────────────────────────────────────────────────
%  LEGEND
% ────────────────────────────────────────────────────────────────────────────
\node[above right=0.3cm and 0.5cm of trainbox.north east,
      anchor=north west] (legend) {%
  \begin{tikzpicture}[every node/.style={font=\scriptsize}]
    \node[dataset,  minimum width=1.3cm, text width=1.3cm,
          minimum height=0.45cm] at (0,0)    {\strut Data};
    \node[prompt,   minimum width=1.3cm, text width=1.3cm,
          minimum height=0.45cm] at (0,-0.70) {\strut Prompting};
    \node[llm,      minimum width=1.3cm, text width=1.3cm,
          minimum height=0.45cm] at (0,-1.40) {\strut LLM};
    \node[vector,   minimum width=1.3cm, text width=1.3cm,
          minimum height=0.45cm] at (0,-2.10) {\strut Vector op.};
    \node[layersel, minimum width=1.3cm, text width=1.3cm,
          minimum height=0.45cm] at (0,-2.80) {\strut Layer sel.};
    \node[mlp,      minimum width=1.3cm, text width=1.3cm,
          minimum height=0.45cm] at (0,-3.50) {\strut MLP};
    \draw[darrow, gray] (0.1,-4.3) -- ++(1.1,0)
      node[right] {transfer};
  \end{tikzpicture}
};

\end{tikzpicture}
